Wasserstein Distances, Neuronal Entanglement, and Sparsity

Disentangling polysemantic neurons is at the core of many current approaches to interpretability of large language models. Here we attempt to study how disentanglement can be used to understand performance, particularly under weight sparsity, a leading post-training optimization technique. We suggest a novel measure for estimating neuronal entanglement: the Wasserstein distance of a neuron's output distribution to a Gaussian. Moreover, we show the existence of a small number of highly entangled "Wasserstein Neurons" in each linear layer of an LLM, characterized by their highly non-Gaussian output distributions, their role in mapping similar inputs to dissimilar outputs, and their significant impact on model accuracy. To study these phenomena, we propose a new experimental framework for disentangling polysemantic neurons. Our framework separates each layer's inputs to create a mixture of experts where each neuron's output is computed by a mixture of neurons of lower Wasserstein distance, each better at maintaining accuracy when sparsified without retraining. We provide strong evidence that this is because the mixture of sparse experts is effectively disentangling the input-output relationship of individual neurons, in particular the difficult Wasserstein neurons.

==> guidelines.tex <==
\section{Submission of conference papers to ICLR 2025}

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NeurIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2025 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available online at:
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2025_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2025_conference.sty+ and \verb+iclr2025_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2025_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.


There will be a strict upper limit of 10 pages for the main text of the initial submission, with unlimited additional pages for citations. 

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

==> sections/Checklist.tex <==
% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The main claims made in the abstract and introduction are substantiated by well-designed empirical experiments. The contributions of the paper are systematically detailed, particularly in sections 3, 4, and 5, where each aspect is thoroughly explored and supported by the experimental results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: In the discussion and conclusion, we discuss the key limitations of our study, which we aim to address in following studies.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper is centered around empirical experiments, and we do not include theoretical results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper fully discloses all the necessary information to reproduce the main experimental results. Section 5 provides a comprehensive description of the experiments, enabling a careful reader to replicate the results without needing the authors' code. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper utilizes publicly available LLM datasets for training and evaluation. The authors plan to release all code, along with detailed instructions, as open-access to the scientific community upon publication. The paper already includes sufficient instructions to ensure that the main experimental results can be faithfully reproduced. Additionally, the authors are willing to share an anonymized version of the codebase upon request.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper specifies all the necessary training and test details to understand the results. At the beginning of Section 5, we provide comprehensive information about the models, datasets, and experimental environment used in this study. Additionally, we include all necessary benchmarking details to ensure that readers can easily follow and replicate our results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Unfortunately, we were unable to conduct multiple trials for each of our experiments, as they spanned across multiple models and settings for each model. Collecting replicates for each experiment would have been highly computationally expensive. However, we focus on analyzing the results of each conducted experiment in depth to verify their accuracy.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  In the beginning of Section 5, we provide the details of models, dataset, and experimental environment aimed at providing details about the resources required to reproduce the experimental results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The research conducted in the paper conforms, in every respect, with the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper discusses the positive societal and environmental impacts of the work performed. We do not believe that there are any significant negative societal impacts associated with LLM compression and LLM interpretability.
    % In our view, there are little to no negative societal  impacts of LLM compression and interperability research. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not release any novel models or data as part of the submission. The implementations we provide do not have associated risks to be considered placing safeguards for.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The two family of open LLMs Llama and Pythia are properly credited and cited in the paper. The models license and terms of use are mentioned in Section 5.1.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No new assets are introduced in the paper (including code) in the current submission phase. However, we are happy to provide an anonymized codebase upon request for review.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing or human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This study does not involve human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> sections/Discussion_old.tex <==
In this work, we have shown for the first time the role of entanglement, and in particular of highly entangled neurons, in the accuracy of computing the FFN blocks of LLMs. 
%Perhaps, just as outlier features and weights are well understood to be one of the most significant challenges when quantizing to fewer bits \citep{kim2023squeezellm, dettmers2022gpt3, ashkboos2024quarot, egiazarian2024extreme, dettmers2023spqr, zhao2023atom}, neuronal entanglement can provide a path to understanding the challenge of pruning to higher sparsities. 
We have shown that the Wasserstein distance between the output distributions of neurons and the Gaussian distribution is a very suitable metric to identify the degree of entanglement in different neurons. Furthermore, we demonstrated the relevance of highly entangled neurons in the performance of models, both in terms of differentiating between similar inputs and in their significant sensitivity to sparsification and compression. As the focus of our study is analytical, we have only shown per-layer inference speeds. 
In future work, we plan to integrate with an inference framework such as HuggingFace Transformers to show end-to-end inference numbers. We also plan to integrate with MoE-specific inference optimizations such as~\cite{eliseev2023fast}, which should be compatible with our approach as well. 

%To alleviate the difficult nature of sparsifying highly entangled neurons, we introduced a new post-training sparsification scheme, {\mymethod}. As {\mymethod} is based upon the SparseGPT algorithm, it too performs sparsification in one-shot without expensive retraining. In our evaluations, {\mymethod} achieves state of the art performance across all sparsification and compression conditions and across all models tested. Furthermore, it transforms the highly complex output distributions of entangled neurons into easier to model, more Gaussian component distributions. Thus, higher sparsity can be achieved. 
Looking forward, perhaps, just as outlier features and weights are well understood to be one of the most significant challenges when quantizing to fewer bits \citep{kim2023squeezellm, dettmers2022gpt3, ashkboos2024quarot, egiazarian2024extreme, dettmers2023spqr, zhao2023atom}, neuronal entanglement can provide a path to understanding the challenge of pruning to higher sparsities. 

% Quantization is a parallel and complementary model compression technique to sparsification. It operates by representing individual weights with fewer bits, thereby decreasing training and inference cost. It is well known that one of the most significant challenges with quantization to fewer bits is the presence of outlier weights \citep{kim2023squeezellm} and features \citep{dettmers2022gpt3}, in terms of their magnitude. As fewer possible weights are allowed, the presence of the outliers force the weights to be "stretched" over a greater range, reducing their fidelity to the original weights. Many techniques, such as QuaRot \citep{ashkboos2024quarot}, AQLM \citep{egiazarian2024extreme}, SqPR \citep{dettmers2023spqr}, and Atom \citep{zhao2023atom} all attempt to address these outliers via different methods.

% To our knowledge, there is much less understanding regarding the difficulty in sparsifying networks to high sparsities, especially in LLMs. It has been observed that at higher sparsities, model performance drops off sharply in LLMs \citep{jaiswal2024emergence}, and that certain weights that highly correspond with input features are favored to remain at higher sparsities \citep{lee2018snip}. However, unlike with the effects of outliers for quantization, there is still no clear reason for this performance drop off. We hope the entanglement of neurons and its role in sensitivity to pruning begins to provide a path to understanding this phenomena.

%\noindent\textbf{Limitations and Future Work.}
%We believe that there is still significant room to explore the significance of highly entangled neurons in LLMs. We have demonstrated some of their computational abilities and their relevance to sparsity, we think that they have relevance to LLMs, in particular MoEs, vastly beyond what we show. 
%In our context, the most appealing next question is what happens to highly entangled neurons, and with them to sparse entanglement, as we fine-tune the experts after one-shot sparsification. 

%As the focus of our study is analytical, we have only shown per-layer inference speeds. 
%In future work, we plan to integrate with an inference framework such as HuggingFace Transformers to show end-to-end inference numbers. We also plan to integrate with MoE-specific inference optimizations such as~\cite{eliseev2023fast}, which should be compatible with our approach as well. 

%  However, a significant number of weight indices are shared among the different clusters. If all of those weights were collapsed into one matrix, then this matrix could be shared among all inputs. In this way, the same "base" expert could be run for all inputs at the same time, and a much smaller sized "specialization" expert could be run for each input. Throughput could also be optimized in this implementation, where routing to and computation with the specialized experts for each input would be run in parallel with the global computation with the base expert matrix. However, as all the weights in the same indices across clusters are still different, a small amount of fine-tuning may be necessary. 


==> sections/Introduction_old.tex <==
% From mitthesis package
% Version: 1.04, 2023/10/19
% Documentation: https://ctan.org/pkg/mitthesis

The past few years have seen an explosion in machine learning model capabilities, specifically  those of transformers and large language models (LLMs). 

Interpretability of model behavior has been a longstanding goal of machine learning research \ling{cite}. One of the related concepts of polysemanticity and superposition. Neurons activating for a set of unrelated concepts has been an obstacle to advances in the mechanistic interpretability of LLMs. Even though there is a plethora of ongoing research contributing to the understanding of polysemanticity and superposition in neural networks \shashata{cite}, there is still a gap in determining the extent of neuron polysemanticity. 

However, such an increase in capability has demanded an exponential increase in model size, incurring drastic monetary and energy costs.

The performance of LLMs is dominated by the number of parameters executed per input token during computation, both due to the number of multiply-add (FMA) operations required per parameter, and data movement to set up these operations. Neural network sparsity \citep{hoefler2021sparsity} attempts to reduce the executed number of parameters and thus improve performance.  The most common form of sparsity is static sparsification, wherein unnecessary model parameters are pruned away, and the model performs the same computation for every input. Many methods, such as gradual magnitude pruning \citep{zhu2017prune}, Wanda \citep{sun2023simple}, and SparseGPT \citep{frantar2023sparsegpt}, utilize this approach. SparseGPT, in particular, is the state-of-the-art one-shot pruning technique, allowing models to be  cheaply compressed without expensive retraining.

In contrast, input-dynamic sparsity involves performing different computations on different inputs and is generally achieved through converting a dense model into a mixture of experts (MoE) like framework. Existing techniques, including DejaVu \citep{liu2023deja}, MoEification \citep{zhang2021moefication}, and Scaling Transformers \citep{jaszczur2021sparse}, route inputs only to computations predicted to be necessary. These methods are based on the sparsity induced by the ReLU activation function and cannot be easily extended to other popular activation functions such as GeLU (as in GPT models~\citep{radford2018improving}) and SwiGLU (as in Llama \citep{touvron2023llama}). 
% [[move to related work]]] Recently, other approaches have attempted to impart activation sparsity to non-ReLU models by converting their activation functions to ReLU, as is the case with Relufication \citep{mirzadeh2023relu}, or to directly threshold post-activation function values based on magnitude, as is the case with CATS \citep{lee2024cats}. However, the former approach requires expensive retraining, and the latter requires one linear layer in each feedforward network (FFN) block to be run densely.

In this paper, we improve the one-shot sparsification of a model by expanding it into a mixture of experts, where each expert is a copy of the original, statically pruned to perform well on a subset of the inputs. Our technique, which we dub {\mymethod}, 
begins by clustering input embeddings layer-wise; based on this clustering, {\mymethod} leverages the input-aware nature of the SparseGPT pruner to specialize different sparse experts to different sets of inputs, starting from the same base weights. At run time {\mymethod} routes the inputs to the sparse experts at each layer based on the clustering (one could of course use more a sophisticated MoE router \cite{zhang2021moefication} in place of clustering). Our approach increases the overall size of the model, but greatly reduces the number of executed run time parameters. Through {\mymethod}, we achieve state-of-the-art one-shot sparsification performance in terms of %non-zero 
parameters activated per token, across LLMs from the Llama and Pythia families, at low accuracy loss. Moreover, we show that our approach can be coupled with efficient execution kernels, leading to non-trivial speedups for generative inference; for the largest linear layers in Llama 2 7B and 70B, a variant of our approach provides speedups of 3x and 4.8x, respectively, even  taking the expert routing overhead into account.   
% To avoid expensive retraining and being limited to ReLU-based models, we utilize one-shot sparse expert creation in every FFN block linear layer. 

Our main technical contribution is a detailed study of how this expansion method obtains performance. Every neuron in a network has a certain level of ``entanglement,'' which we view as the degree to which it must deal with different combinations of features in its inputs. We observe for the first time the existence of ``highly entangled'' neurons in the dense model. These neurons, which appear in all model layers, have striking, irregular output distributions (Figure \ref{fig:clustering_saves_llama}d), and as we show later, seem to be responsible for the difficult task of differentiating similar input vectors through their dot product computation. Furthermore, these neurons have an outsize effect on model performance: removing them increases error much more than a similar collection of random neurons (Figure \ref{fig:high_WD_sensitivitiy}). We found that one can quantify the degree to which a neuron is entangled via the Wasserstein distance \citep{kantorovich2006translocation} between its output distribution and a properly-normalized Gaussian. 

Sparsity tends to push the outputs of a dot-product of a neuron towards the Gaussian distribution as it loses edges (see Figure \ref{fig:high_sparsity}), even with an adjustment of edge weights. It thus reduces the expressive power of each neuron, and leads to increased error. In accordance, high Wasserstein distance neurons are particularly difficult to sparsify, especially at higher sparsities.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{sections/figures/clustering_saves_llama.png}
    \caption{The output distributions of neurons in Llama 2 7B. One can see that the red {\mymethod} output distribution covers a random neuron slightly better than than the green SparseGPT distribution, and this improvement becomes much more pronounced for an entangled neuron. The reason is the ability of the separate dot product operations of the multiple experts, depicted each in a separate color (in c and f), to better cover the dense distribution. Sparsity is set to 90\% per expert and the neurons are from the gate projection of the second FFN block. WD is the Wasserstein distance between the {\mymethod} sparse output distribution and the dense distribution. RI is the relative improvement of {\mymethod} over SparseGPT, defined later.}
\label{fig:clustering_saves_llama}
\end{figure}

We provide evidence that the key to the performance of {\mymethod} is that it effectively ``disentangles'' the neuronal output distributions, in particular those with high Wasserstein distances, into much simpler ones. For example, SparseGPT mostly succeeds in capturing the dense output distribution of a non-entangled neuron with a sparse one (Figure \ref{fig:clustering_saves_llama}a). However, it fails to capture the full dense output distribution of a highly entangled neuron (Figure \ref{fig:clustering_saves_llama}d). {\mymethod} overcomes this by disentangling the neuron. Each sparse expert is responsible only for a clustered subset of the inputs (i.e. can be viewed as capturing a subset of the input features) allowing it to model these with the more Gaussian shaped distribution imposed by sparsity. Each neuron's output is then modeled by the collection of outputs of all the experts together. While sparse disentanglement helps cover the normal neuron's distribution slightly better than SparseGPT, it greatly helps it in covering the output distribution of the entangled neuron where SparseGPT fails (Figure \ref{fig:clustering_saves_llama}f). The {\mymethod} technique allows one to readily see this because, unlike in traditional MoEs, each neuron retains the exact same position and role in each of the experts.

% see Figure \ref{fig:clustering_saves_llama}, where (above left) we see how SparseGPT mostly succeeds in capturing the output distribution of a dense neuron with a sparse one, while it fails to capture the full output distribution of a dense high Wasserstein neuron (below left) with a sparse one. However, {\mymethod} overcomes this by disentangling the neuron. Each sparse expert is responsible only for a clustered subset of the inputs (i.e. can be viewed as capturing a subset of the input features) allowing it to model these with the more Gaussian shaped distribution imposed by sparsity. Each neuron's output is then modeled by the collection of outputs of all the experts together. In the middle of Figure \ref{fig:clustering_saves_llama}, one can see that while sparse disentanglement helps cover the normal neuron's distribution (above middle) a bit better than sparseGPT (above right), it greatly helps it in covering the Wasserstein neuron (below middle) where sparseGPT (above right) fails. The {\mymethod} technique allows one to readily see this because, unlike in traditional MoEs, each neuron retains the exact same position and role in each of the experts. 


Because {\mymethod} effectively disentangles neurons throughout the model, it improves its overall sparse performance, and not surprisingly, as the number of experts applied to a model grows, and with it its ability to disentangle, the overall accuracy of {\mymethod} improves (Figure \suppfigref{fig:more_clusters}). 

Finally, we note that in the literature, disentanglement is generally used in the context of mechanistic interpretability to generate human-understandable features \citep{elhage2022toy, higgins2017beta}. Here, we use disentanglement as a performance enhancing tool, and link it to improved performance via induced sparsity. We believe this phenomena is at the base of general MoE performance, but is harder to analyze because of the retraining of the experts. 

In the next section we explain the implementation of {\mymethod} in detail. We then study how it supports  disentanglement in LLMs, and finally present  results showing its performance relative to other state of the art one-shot compression techniques. 





==> sections/Method.tex <==
\label{sec:methods}



% \subsection{\mymethod}

\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{sections/figures/Sparse_Expansion.png}
    \caption{The {\mymethod} process. One-shot expert creation process of {\mymethod} (left). Inference process in an FFN block of {\mymethod} (right).}
    \label{fig:DiCE creation}
\end{figure}

At a high level, {\mymethod} clusters the incoming inputs to each layer into separate groups. Then, each expert is sparsified via the SparseGPT pruning algorithm~\citep{frantar2023sparsegpt}. Briefly, SparseGPT approximates the optimal sparse version w.r.t. L2 distance relative to the dense outputs of a given layer by leveraging the Hessian matrix of the second order derivatives of the error relative to the parameters within each linear layer $\mathbf{y = WX + b}$. Here, $\mathbf{y}$ is the set of outputs of the layer, $\mathbf{W}$ is the weight matrix for the layer, $\mathbf{b}$ is the bias for the layer, and $\mathbf{X}$ is a set of inputs arranged as a matrix, where each column is a separate input vector. Doing so yields $\mathbf{H = XX^T}$, where $\mathbf{H}$ is the Hessian matrix. Furthermore, SparseGPT is natively capable of performing one-shot quantization as well, due to the sharing of the error updates between sparsification and quantization. In our experiments, we thus test {\mymethod} in both sparse and joint sparse-quantized settings.

% In Sparse Expansion, because we separate the inputs into different clusters, a unique Hessian matrix can be calculated for each cluster. We thus generate a mixture of sparse experts in one-shot from a standard dense model.

In Sparse Expansion, we leverage the observation that  SparseGPT is input-aware, and cluster the inputs to each layer via K-means and designating a separate, initially identical, expert for every cluster of inputs. (In order to facilitate better and faster clustering, we first utilize principal  component analysis (PCA) to reduce the dimensionality of the inputs.) Following the clustering of the inputs, each sparse expert can now be tailored to a subset of inputs rather than trying to adapt to all of them. To allow the experts to specialize, a separate Hessian matrix is calculated for every input cluster, which is then used to prune the expert weight matrix through the SparseGPT pruning algorithm. Specialized experts have now been generated that are adapted to the subset of inputs routed to the corresponding cluster (Figure \ref{fig:DiCE creation}, Algorithm \suppalgref{alg:modelgen}). Our {\mymethod} approach therefore yields a mixture of sparse experts through one-shot sparsification, removing the need for expensive retraining.

During inference, each input will first have its dimensionality reduced by the PCA model, then separately evaluated via the K-means model to decide its expert, and finally be routed to the corresponding expert for the matrix multiply (Algorithm \suppalgref{alg:modelinf}). As the routing is done via K-means on a lower dimension, and the PCA is a very low dimension matrix multiply, both are inexpensive to add on to normal LLM inference. Furthermore, routing in this manner prevents the need to train and run a more expensive router. 

Our design departs from traditional MoEs in terms of their routing for the benefit of sparsity. In traditional MoEs, inputs are generally routed at the start of each FFN block once, such that the same up, gate, and down projection experts are associated with a particular routing. Furthermore, inputs are generally routed to multiple experts per inference pass, thus increasing the effective number of experts through the combination of different ones. However, routing to multiple experts in our case would incur a penalty in the sparsity of the model. Thus, we instead chose to do routing for the up and gate projection experts, and then again for the down projection expert (\ref{fig:DiCE creation}). In this way, we square the effective number of experts combinations per input to a FFN block without decreasing sparsity.



% \subsection{Neuron-based Analysis}
% To fully understand how {\mymethod} improves upon a static sparsification scheme, we will investigate the output distributions at the per neuron level. We will determine which clustered neurons improve the most over their static counterparts, and also explore what characteristics such neurons share. Finally, we will explore the distributions of the individual clusters as well.

==> sections/Result_old.tex <==
\section{Neuronal disentanglement}

% Disentanglement is most often regarded as a process of training a model in a way such that features are encoded in an interpretable manner \citep{higgins2017beta}. It is related to the concept of feature superposition, wherein a neural network is able to encode more such features than it has dimensions, due to the features being sparsely present \citep{elhage2022toy}. Both are sub-fields in the larger realm of mechanistic interpretability, which aims to explain the computational trajectory of models in an understandable manner \citep{molnar2020interpretable}.

% However, here we envision disentanglement differently, on the level of neuronal computation. Rather than operate in the space of reframing features learned by a network into individually human interpretable features, we instead operate in the space of decomposing the output distributions of an linear layer into simpler component distributions on the single neuron level. Specifically, we examine how different neurons are responsible for different output distributions through their inner product computations, and the relative difficultly between modeling such output distributions in a sparse setting. We investigate how output distributions are separated - disentangled - into more simple component distributions through clustering of the inputs, and to what degree the clustering improves performance.


\subsection{Characterizing non-Gaussian neuronal output distributions}
We investigate the output distributions of individual neurons as the model processes its inputs during inference across all linear layers in each transformer block feed forward network (FFN). We focus our analysis in Pythia 1.4B \citep{biderman2023pythia} and Llama 2 7B \citep{touvron2023llama}. Most neurons exhibit a reasonably Gaussian output distribution after their dot product operation on the input vector (Figure \ref{fig:neuron_output_IO}a, \ref{fig:clustering_saves_llama}a). However, we find the existence of a small group neurons with highly non-Gaussian outputs (Figure \ref{fig:neuron_output_IO}c, \ref{fig:clustering_saves_llama}c). We observe the existence of such neurons in all FFN blocks of transformers.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.4\linewidth]{sections/figures/sample_diff.png}\includegraphics[width=0.4\linewidth]{sections/figures/cosine_sim_vs_output.png}
%     % \includegraphics[width=0.4\linewidth]{sections/figures/sample_diff_llama.png}
%     \caption{Example neurons' output distributions in Pythia 410M (left) and Llama 2 7B (right). Both the normal (blue) and strange (yellow) neuron's distributions were taken from the up projection matrix in the second FFN block.}
%     \label{fig:weird_neuron_example}
%     \label{fig:weird_neuron_example_llama}
% \end{figure}
\label{sec:WD_method}
To characterize the degree of difference between the non-Gaussian output distributions of these neurons from the Gaussian-like output distribution of an average neuron, we considered several metrics. However, we ultimately chose the Wasserstein distance (WD) \citep{kantorovich2006translocation, villani2009optimal} as a means of quantifying the degree of difference. In optimal transport theory, the WD measures the minimal transportation cost between two distributions, taking their geometry in real space into account. 


% Unlike L1, L2 or Hellinger distances, it captures the true dissimilarity in various metric spaces, making it versatile for complex data structures and distribution shapes. one characterization of the difference between two distributions is known as the Wasserstein Distance \citep{kantorovich2006translocation, villani2009optimal}. 

To find the WD of every neuron to the Gaussian $\mathcal{N}$, we first normalize the output distributions of each neuron $n$ to have zero mean and unit variance, and compare this normalized distribution $n'$ to $\mathcal{N}(0, 1)$. This is because the range of neurons is quite variable, and we wanted to prioritize finding the differences in the shape of the output distribution, not other properties of the distribution. We use the $1$-Wasserstein distance in one dimension, as shown in Equation \ref{eqn:wasserstein_1}: 

\begin{equation}
    W_1(n', \mathcal{N}) = \int_0^1|F^{-1}(z) - G^{-1}(z)|dz.
    \label{eqn:wasserstein_1}
\end{equation}

% The Wasserstein Distance is essentially the amount of work that is required to convert one distribution into another. 
% Formally, from the perspective of optimal transport, it is characterized as the minimum effort required to morph one distribution into another in a metric space. For distributions $\mu$ and $\nu$ on $\mathbb{R}^n$, and employing the Euclidean norm $\|\cdot\|$ as the distance metric, the $p$-Wasserstein distance is defined as: 
% \begin{equation}
% \label{eqn:wasser}
% W_p(\mu, \nu) = \left( \inf_{\gamma \in \Gamma(\mu, \nu)} \int_{\mathbb{R}^n \times \mathbb{R}^n} \|x-y\|^p \, d\gamma(x,y) \right)^{1/p}
% \end{equation}
  
% \ling{Just use the 1D WD formulation for our use, deviation from normal}

% Here, $x$ and $y$ are points in $\mathbb{R}^n$, $\|\cdot\|$ denotes the norm in $\mathbb{R}^n$, and $\gamma$ represents a transport plan—a joint distribution whose marginals are $\mu$ and $\nu$. The set $\Gamma(\mu, \nu)$ includes all such possible transport plans. This formulation reflects the minimum 'work' needed to transform the distribution $\mu$ into $\nu$, where 'work' is measured by the expected value of the $p$-th power of the distances $\|x-y\|$ over the transport plan $\gamma$.  We use the $1$-Wasserstein distance in one dimension, so $p = n = 1$. Our formula thus simplifies to the equation in equation  \ref{eqn:wasserstein_1}. $F^{-1}$ and $G^{-1}$ represent the inverse cumulative distribution function of $\mu$ and $\nu$, respectively, which can be  approximated with our empirical data.


% \begin{equation}
%     W_1(\mu, \nu) = \int_0^1|F^{-1}(z) - G^{-1}(z)|dz.
%     \label{eqn:wasserstein_1}
% \end{equation}

% To find the Wasserstein distance of every neuron, we first normalize the output distributions of each neuron to have zero mean and unit variance, and compare this normalized distribution to a Gaussian with the same mean and variance. This is because the range of neurons is quite variable, and we wanted to prioritize finding the differences in the shape of the output distribution, not other properties of the distribution.

% \subsection{Selection of Wasserstein Distance as a Metric}
% In optimal transport theory, one characterization of the difference between two distributions is known as the Wasserstein Distance \citep{kantorovich2006translocation, villani2009optimal}. The WD measures the minimal transportation cost between them, providing a robust measure even in the presence of noise and outliers. Furthermore, it is sensitive to the geometry of the data distributions themselves in the real distribution space. Thus, it captures the true dissimilarity across distributions. 

% Formally, from the perspective of optimal transport, the WD is characterized as the minimum effort required to morph one distribution into another in a metric space. For distributions $\mu$ and $\nu$ on $\mathbb{R}^n$, and employing the Euclidean norm $\|\cdot\|$ as the distance metric, the $p$-Wasserstein distance is defined as shown in Figure \ref{fig:wasserstein}.

% \begin{figure}[h]
%   \centering
%     \begin{equation}
%     W_p(\mu, \nu) = \left( \inf_{\gamma \in \Gamma(\mu, \nu)} \int_{\mathbb{R}^n \times \mathbb{R}^n} \|x-y\|^p \, d\gamma(x,y) \right)^{1/p}
%     \end{equation}
%   \caption{The general $p$-Wasserstein distance.}
%   \label{fig:wasserstein}
% \end{figure}

% Here, $x$ and $y$ are points in $\mathbb{R}^n$, $\|\cdot\|$ denotes the norm in $\mathbb{R}^n$, and $\gamma$ represents a transport plan—a joint distribution whose marginals are $\mu$ and $\nu$. The set $\Gamma(\mu, \nu)$ includes all such possible transport plans. This formulation reflects the minimum "work" needed to transform the distribution $\mu$ into $\nu$, where work is measured by the expected value of the $p$-th power of the distances $\|x-y\|$ over the transport plan $\gamma$ \citep{kolourioptimal}. We use the $1$-Wasserstein distance in one dimension, so $p = n = 1$. Our formula thus simplifies to the equation in Figure \ref{fig:wasserstein_1}. $F^{-1}$ and $G^{-1}$ represent the inverse cumulative distribution function of $\mu$ and $\nu$, respectively, which can be easily approximated with our empirical data.

% \begin{figure}[h]
%   \centering
%     \begin{equation}
%     W_1(\mu, \nu) = \int_0^1|F^{-1}(z) - G^{-1}(z)|dz
%     \end{equation}
%   \caption{The $1$-Wasserstein distance in $\mathbb{R}$.}
%   \label{fig:wasserstein_1}
% \end{figure}

% Specifically for our analysis, the WD satisfies the crucial criteria that the metric must take distance in the output space into account. As an exmaple, consider two Gaussian distributions, $A$ and $B$, that each have zero mean and unit variance. A small amount, 10\% of the original number of samples, is added to both $A$ and $B$. These samples also are a Gaussian distribution with unit variance. In $A$, these samples are added with mean 8, and in $B$, these samples are added at mean 12 (Figure \ref{fig:KL_vs_WD}). The metric that we choose should indicate that the difference between distribution $A$ and $\mathcal{N}(0, 1)$ is significantly smaller than the difference between distribution $B$ and $\mathcal{N}(0, 1)$. However, for metrics like Kullback-Leibler (KL) divergence, the two differences are nearly identical, with values of 82, while the comparison with $A$ has a WD of 0.73, and the comparison with $B$ has a WD of 1.09.

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=0.5\linewidth]{sections/figures/KL_vs_WD.png}
%     \caption{The WD metric best captures the differences in the distribution that we are interested in. The metric should indicate that the difference between $A$ and $\mathcal{N}(0, 1)$ is greater than the difference between $B$ and $\mathcal{N}(0, 1)$. Indeed, WD greatly distinguishes between the two differences, while KL divergence does not.}
%     \label{fig:KL_vs_WD}
% \end{figure}

$F^{-1}$ and $G^{-1}$ represent the inverse cumulative distribution function of $n'$ and $\mathcal{N}(0, 1)$, respectively, which can be approximated with our empirical data. To compute the WD of every neuron efficiently, we use the implementation provided by \texttt{SciPy} \citep{virtanen2020scipy}.
When computing the difference metric in this way, we find that our originally observed neurons have been designated correctly with high WD to $\mathcal{N}$. 

% In the two neurons shown for Pythia 410M (Figure \ref{fig:weird_neuron_example}), the neuron on the left has a Wasserstein distance to normal of $0.055$ and the neuron on the right has a distance of $0.406$. In the two neurons shown for Llama 2 7B (Figure \ref{fig:weird_neuron_example_llama}), the neuron on the left has a Wasserstein distance to normal of $0.051$ and the neuron on the right has a distance of $0.408$. We will continue to use these same four neurons as illustrative examples. Furthermore, we find neurons with a high Wasserstein distance to normal (high WD neurons) in all up and gate projection layers, and some down projection layers (Figure \suppfigref{fig:WD_in_all}), and the high WD neurons have the odd shapes that we have been observing.

% \subsection{Importance of High Wasserstein Neurons in Model Performance}

\subsection{Wasserstein distances and entanglement}

All neurons in the models we examined show some non-zero WD, and yet we find neurons with a high WD in all up and gate projection layers, some down projection layers (Figure \suppfigref{fig:WD_in_all}) in Llama 2 7B. Henceforth we focus on the high WD neurons because they offer a clearer example of the correlation of the WD with the computational roles of neurons. The high WD neurons have the odd shapes that we have been observing (Figures \suppfigref{fig:neuron-llama-top-30} and \suppfigref{fig:neuron-pythia-top-30}). We consider the difficulty of the dot product computation neurons perform in terms of the input-output relationships they are expected to handle in four broad groups. Namely, the dot product may map similar inputs to similar outputs, dissimilar inputs to dissimilar outputs, dissimilar inputs to similar outputs, and similar inputs to dissimilar outputs. Of the four relationships, the last seems most difficult to model, as small changes in the inputs must be mapped far away in output space. This relationship would be even more difficult to maintain under sparsity. This is because, as the number of nonzero entries in the weight vector decrease, the means and variance both tend toward zero (Figure \suppfigref{fig:mean_var_zero}). Such a setting makes it all the more difficult to keep similar inputs far apart in the output space.
% Between pairs of inputs to a neuron, and their associated outputs after the dot product is applied through the neuron's weight vector, there are four general input-output relationships between pairs of inputs and pairs of outputs. 
% First, a pair of similar inputs may get mapped to similar outputs. Next, a pair of dissimilar inputs may get mapped to dissimilar outputs. Next, a pair of dissimilar pair of close inputs may get mapped to a pair of similar outputs. Finally, a pair of similar inputs may get mapped to a pair of dissimilar outputs. 

% latter two seem the most difficult to model, as large changes in the inputs lead to small changes in the outputs, and vice versa, respectively. Furthermore, under a sparse setting, the last relationship where similar inputs are mapped to dissimilar outputs is likely the most difficult to maintain. This is because, as the number of nonzero entries in the weight vector decrease, the means and variance both tend toward zero. Such a setting makes it all the more difficult to keep similar inputs far apart in the output space.

We use cosine similarity to measure the similarity between inputs and L1 distance to measure the similarity between outputs following computation by a particular neuron's dot product. Larger cosine similarities indicate more similar inputs, and smaller L1 distances indicate more similar outputs. In Pythia 1.4B, for a neuron with a normal output distribution, the relationship between its input-output pairs is fairly reasonable. Very similar inputs with a cosine similarity of close to one have very similar outputs with L1 distance close to zero. Unrelated inputs with cosine similarity of close to zero have very far outputs with a large L1 distance between them. As input similarity decreases, output distance increases. Finally, there are pairs of dissimilar inputs that are mapped to close values. However, there are no input pairs that are similar with highly dissimilar outputs (Figure \ref{fig:neuron_output_IO}b).

However, for a high WD neuron, \emph{this is not the case}---in addition to the previously mentioned relationships, it now has to contend with discerning between two similar inputs and map them far away in output space (Figure \ref{fig:neuron_output_IO}d). Note that even for two inputs that share a cosine similarity of 0.9, this neuron sometimes has to map them across a majority of its entire effective range.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{sections/figures/neuron_output_IO.png}
    % \includegraphics[width=0.4\linewidth] {sections/figures/cosine_sim_vs_output_llama.png}
    \caption{Neuronal entanglement. The high WD neuron must map fairly similar inputs to outputs that are very far apart (as indicated by the dense upper right hand corner of (d) vs the empty one in (b)) through its dot product operation. The neurons are from the up projection of the second FFN block in Pythia 1.4B.}
    \label{fig:neuron_output_IO}
\end{figure}

% For Llama 2 7B, the overall shape of the pairwise relationship is different, but the trend still holds. In the normal neuron, similar inputs get mapped to similar outputs, and dissimilar ones to dissimilar ones. Interestingly, there are fewer intermediately similar inputs being mapped to intermediately similar outputs. However, in the high WD neurons, as before, more similar inputs, this time having around a cosine similarity of 0.5, are being mapped great distances apart (Figure \ref{fig:cosine_sim_output}).

% We therefore term these neurons with output distributions that have a high Wasserstein distance from the Gaussian distribution as "entangled". This is because inputs that must be mapped far away in output space are close by and entangled in the input space. 

Because inputs that must be mapped far away in output space are close by and entangled in input space, we therefore term these high WD neurons as ``entangled.''

\subsection{Effect of high Wasserstein neurons on sparsification}

We show that entangled neurons have a substantially outsized effect on model performance through the lens of sparsity. In Llama 2 7B, if just the 3\% of the highest WD neurons are sparsified in every FFN block, model performance significantly degrades, far more than if random neurons were sparsified. The same is true if the neurons are sparsified 2:4 and then quantized to fewer bits, with high WD neurons drastically inhibiting model performance under compression. As compression increases, this effect becomes more obvious (Figure \ref{fig:high_WD_sensitivitiy}). Therefore, entangled neurons are crucial for maintaining model accuracy and are severely limited in their ability to be compressed.
% If just the 3\% of neurons that have the highest WD are sparsified, In Llama 2 7B, in every projection matrix of every FFN block, 3\% of neurons were chosen, either the neurons with the highest WD or at random. These neurons were either sparsified to the same percentage in an unstructured manner, or sparsified to 2:4 and then quantized, both through SparseGPT. Compressing these high WD neurons, both through the level of sparsity and the number of bits, significantly hampers the model, moreso than compressing random neurons. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{sections/figures/highWDsensitivity.png}
    \caption{Entangled neurons are sensitive to compression. In Llama 2 7B, 3\% of neurons from every layer were sparsified in an unstructured manner (left) or sparsified to 2:4 and quantized (right). Compressing high WD neurons impairs the model significantly more than compressing random ones.}
    \label{fig:high_WD_sensitivitiy}
\end{figure}

Additionally, as a neuron is increasingly sparsified, the output distribution becomes more Gaussian (See Figure~\ref{fig:high_sparsity}). This in turn places even more stress upon the neuron - not only is it contending with the decreasing mean and variance, but also with the less expressive distribution shape. Thus, it seems that, especially at the higher sparsities that we are investigating, the irregular shape of the entangled neurons is much more challenging to model with fewer weights than a Gaussian-like distribution. To address the difficulty of sparsifying entangled neurons, we introduce {\mymethod}. 
% Furthermore, we investigated how exactly the entangled neurons perform under sparsity. In these experiments, neurons in the up projection matrix in the second FFN block were sparsified using SparseGPT to the same unstructured sparsity per neuron. For Pythia 410M, that was 80\% sparsity, and for Llama 2 7B, that was 90\%. In both cases, random neuron's output distribution shape under sparsity better approximated the dense output distribution compared to the entangled neuron's distribution. This is especially apparent in Pythia 410M, where, as the sparse dot product tries to capture the shape of the output distribution, the range greatly suffers, causing the distribution as a whole to shrink inward. Indeed, the Wasserstein distance between the dense and sparse output distributions in Pythia 410M was 0.08 and 0.17 for the random and entangled neurons, respectively. In Llama 2 7B, the distances were 0.016 and 0.018, respectively (Figures \ref{fig:hard_to_sparsify}, \ref{fig:hard_to_sparsify_llama}). Thus, it seems that, especially at the higher sparsities that we are investigating, the irregular shape of the entangled neurons is much more challenging to model with fewer weights than a Gaussian-like distribution.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{sections/figures/Distribution_of_neurons_with_sparsity.png}
    \caption{Increasing sparsity induces normality. A highly entangled neuron's dense distribution (blue) and sparse distributiuon (red). As sparsity increases, the output distribution of sparse neurons becomes progressively more Gaussian. WD represents the Wasserstein distance. This is the same neuron from Figure \ref{fig:neuron_output_IO}c.}
    \label{fig:high_sparsity}
\end{figure}


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.4\linewidth]{sections/figures/hard_to_sparsify.png}\includegraphics[width=0.4\linewidth]{sections/figures/hard_to_sparsify_llama.png}
%     \caption{The output distribution of the normal neuron is much better modeled under sparsity than the distribution of the entangled neuron is. Note how the whole shape seems to be compressing inward, drastically decreasing the fidelity of the sparse dot product. This is in Pythia 410M.}
%     \label{fig:hard_to_sparsify}
% \end{figure}
\section{{\mymethod} disentangles neurons}
%\subsection{Input Clustering Recovers the Output Distribution of Entangled Neurons}

We revisit the output distributions of neurons to determine the effect that clustering has in a sparse setting. We measure the relative improvement (RI) that {\mymethod} provides, where relative improvement is defined as the ratio of the L2 error between the dense output and the SparseGPT sparse output to the L2 error between the dense output and the {\mymethod} sparse output.  

% For both Llama 2 7B (Figure \ref{fig:clustering_saves_llama}) and Pythia 1.4B (Figure \suppfigref{fig:clustering_saves}), both the random neuron and the entangled neuron improve through {\mymethod}, and the latter improves much more. 
For Llama 2 7B (Figure \ref{fig:clustering_saves_llama}) and Pythia 1.4B (Figure \suppfigref{fig:clustering_saves}), both models and both neuron types—random and entangled—improve through {\mymethod}, with the entangled neuron showing greater improvement. Furthermore, for the random neuron and especially for the entangled neuron, the geometry of the sparse output distribution much more closely matches that of the dense distribution in {\mymethod}.

We also provide a visualization for the specialization of each cluster. Figure \ref{fig:clustering_saves_llama} and Figure \suppfigref{fig:clustering_saves} each show the sparse output distributions of each individual cluster, with a different color per expert. For the randomly selected neurons, there is an improvement though each expert by and large is still responsible for approximately the same range and shape. For the entangled neurons, there is significant specialization for different parts of the distribution further away from the mean. 

However, {\mymethod} is not limited to improving just neurons with a high WD to normal. Across different sparsities and across different models, all but a tiny fraction of neurons improve through {\mymethod} (Figure \suppfigref{fig:improvement_over_sparsity}). Thus, we believe that, in fact, every neuron is to some extent entangled. However, neurons with a high WD are the most obviously entangled neurons, and they benefit more from sparse disentanglement, especially at higher sparsities.

Finally, we note that other metrics of the dense neuronal output distribution, such as their means and variances, fail to act as a predictor of neuronal improvement to the degree that the Wasserstein distance to a Gaussian does (Figure \suppfigref{fig:meanvar}). Thus, we believe the Wasserstein distance to be the most suitable metric of entanglement within a neuron.

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=0.9\linewidth]{sections/figures/clustering_saves_llama.png}
%     \caption{{\mymethod} provides a much better sparse model for entangled neurons in Llama 2 7B. The top row of panels displays a normal neuron, and the bottom row displays an entangled neuron. The dense output distribution is shown in blue behind the SparseGPT sparse distribution in green in the left panel and the {\mymethod} sparse distribution in red in the middle panel. In the right panel, each cluster is shown in a distinct color to visualize its range.}
%     \label{fig:clustering_saves_llama}
% \end{figure}

\subsection{More sparse experts better fit the output distribution}

The complex dense output distribution of highly entangled neurons is difficult to model with a single sparse expert, as in the case of SparseGPT. In figure \ref{fig:moreclusters}, we show the output distribution of a high WD neuron in both dense and sparse computation. As the number of sparse experts increases, the output distribution of the sparse computation more closely matches that of the dense computation, as measured in both WD between the two distributions and relative improvement.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{sections/figures/dense_h_to_4h_cluster_sparse_distribution_neuron_2402_layer_1.png}
    \caption{Modeling recovery with more experts. The sparse computation output distribution (red) matches the dense one (blue) better with more clusters. Sparsity is set to 90\% for each expert. WD represents the Wasserstein distance between the {\mymethod} sparse output distribution and the dense distribution. RI represents relative improvement of Sparse Expansion ($n \geq 1$ clusters) over SparseGPT ($n = 1$ cluster). This is the same neuron from Figure \ref{fig:neuron_output_IO}c.}
    \label{fig:moreclusters}
\end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{sections/figures/high_WD_improve.png}
%     \caption{As sparsity increases, entangled neurons benefit more from clustering. Each blue dot represents a single neuron, with its Wasserstein distance to a Gaussian plotted against its relative improvement from SparseGPT to {\mymethod} as defined before. At lower sparsities, both normal and entangled neurons benefit from clustering, but as sparsity increases, highly entangled neurons benefit much more. These neurons are from the up projection layer in the second FFN block in Pythia 410M.}
%     \label{fig:high_WD_improve}
% \end{figure}

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=\linewidth]{sections/figures/high_WD_improve_llama.png}
%     \caption{As sparsity increases, entangled neurons benefit more from clustering. Each blue dot represents a single neuron, with its Wasserstein distance to a Gaussian plotted against its relative improvement from SparseGPT to {\mymethod} as defined before. At lower sparsities, both normal and entangled neurons benefit from clustering, but as sparsity increases, highly entangled neurons benefit much more. However, this phenomenon occurs at a much higher sparsity than in Pythia 410M. These neurons are from the up projection layer in the second FFN block in Llama 2 7B.}
%     \label{fig:high_WD_improve_llama}
% \end{figure}

\section{{\mymethod} performance}

% \subsection{Setup}


% Wanda\footnotemark\footnotetext{https://github.com/locuslab/wanda}

\subsection{Models, datasets, and setup}

We use the Pythia \cite{biderman2023pythia} series of pre-trained LLMs to evaluate how {\mymethod} performs across model sizes, from Pythia 70M to Pythia 12B. We further evaluate {\mymethod} across the entire Llama 2 family \cite{touvron2023llama2}. We use the Wikitext-2 dataset \cite{merity2016pointer} as calibration data for input-aware pruning and evaluation. For our performance benchmarks, we use 16 clusters at each level of routing in {\mymethod}. For all experiments, we use two NVIDIA A100 Tensor Core GPUs, except for Llama 2-70B where we use three NVIDIA A100s. We rely upon the RAPIDS library \citep{raschka2020machine} to accelerate the fitting and running of the PCA and K-means models by orders of magnitude. To run all models densely and through the MP, Wanda, and SparseGPT pruning approaches, we use a single AMD Instinct MI100 Accelerator GPU. Finally, we utilize and build upon the SparseGPT repositories.

\subsection{Compression across scales}

We evaluate the performance of {\mymethod} against other one-shot pruning techniques across a range of model sizes in Pythia (Figure \ref{fig:scaling_size}). To test both sparsification as well as compression, we compare the pruning techniques when sparsifying each model to 50\% unstructured sparsity, as well as to 2:4 structured sparsity and 3 and 4 bit quantization. Across all model sizes, {\mymethod} outperforms all other pruning techniques, approaching dense performance as model size increases. In fact, for compression, {\mymethod} performs better at 3 bits than SparseGPT does at 4 bits across all model sizes but one.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{sections/figures/scaling_size.png}
    \caption{{\mymethod} across model sizes. Comparisons were made between Magnitude Pruning (MP), Wanda, SparseGPT, and {\mymethod} on the Pythia series of models from sizes of 70M parameters to 12B parameters. Every MLP in each model was sparsified to 50\% sparsity (left) or sparsified 2:4 and quantized to 3 or 4 bits (right). Performance was measured in cross-entropy loss to better show scaling laws.}
    \label{fig:scaling_size}
\end{figure}

\subsection{Performance across sparsification and quantization}

To assess the performance of {\mymethod} at different levels of sparsity or compression for the same model, we compared it to SparseGPT in Llama 2 7B (Figure \ref{fig:scaling_compression}). Every linear layer in each FFN block was sparsified in an unstructured manner across different degrees of sparsity, or sparsified in a structural manner to 2:4 sparsity and then quantized to a different number of bits. Across all levels of sparsity and compression, {\mymethod} performs better than SparseGPT. Furthermore, at higher levels of sparsity and compression, the gap in performance between the two techniques grows. Here as well, {\mymethod} performs better at 3 bits than SparseGPT does at 4 bits.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{sections/figures/scaling_compression.png}
    \caption{{\mymethod} across levels of compression. Comparisons were made between SparseGPT and {\mymethod} on Llama 2 7B. Every layer in each transformer block was sparsified in an unstructured manner (left) or sparsified 2:4 sparsity and quantized to the number of bits (right). {\mymethod} performs the best across all settings as compared to SparseGPT.}
    \label{fig:scaling_compression}
\end{figure}

\subsection{Performance across the Llama family}

Finally, we analyze the performance of {\mymethod} against other sparsification algorithms across all members of the Llama 2 family - Llama 2 7B, Llama 2 13B, and Llama 2 70B - both under sparsity and joint sparsity-quantization compression.

% \begin{table}[h!]
%     \centering
%         \begin{tabular}{| l | c || c | c | c | c |} 
%             \hline
%             & Sparsity & Llama 2 7B & Llama 2 13B & Llama 2 70B & Llama 3 8B \\
%             \hline\hline
%             Dense & 0\% & 5.1168 & 4.5736 & 3.1203 & 5.7503 \\ 
%             \hline
%             MP & 50\% & 16.029 & 6.8270 & 4.9846 & 239.51 \\
%             Wanda & 50\% & 6.7757 & 5.8527 & RUNNING & 8.9281 \\
%             SparseGPT & 50\% & 5.7082 & 5.0521 & 3.6628 & 7.2147 \\
%             {\mymethod} & 50\% & \textbf{5.5839} & \textbf{4.9728} & RUNNING & \textbf{6.9359} \\
%             \hline
%             SparseGPT & 2:4 & 6.9767 & 5.9934 & RUNNING & 9.4381 \\
%             {\mymethod} & 2:4 & \textbf{6.4456} & \textbf{5.6255} & RUNNING & \textbf{8.3346} \\
%             \hline
%         \end{tabular}
%         \caption{{\mymethod} outperforms all other sparsification techniques across the Llama family.}
%         \label{tab:Llama_sparse_performance}
% \end{table}

% \begin{table}[h!]
%     \centering
%         \begin{tabular}{| l | c || c | c | c |} 
%             \hline
%             & Sparsity & Llama 2 7B & Llama 2 13B & Llama 2 70B\\
%             \hline\hline
%             Dense & 0\% & 5.1168 & 4.5736 & 3.3192 \\ 
%             \hline
%             MP & 50\% & 16.029 & 6.8270 & 4.9846\\
%             Wanda & 50\% & 6.7757 & 5.8527 & 4.0219 \\
%             SparseGPT & 50\% & 5.7082 & 5.0521 & 3.9013 \\
%             {\mymethod} & 50\% & \textbf{5.5839} & \textbf{4.9728} & \textbf{3.8791}\\
%             \hline
%             SparseGPT & 2:4 & 6.9767 & 5.9934 & 4.8002\\
%             {\mymethod} & 2:4 & \textbf{6.4456} & \textbf{5.6255} & \textbf{4.6671}\\
%             \hline
%         \end{tabular}
%         \caption{{\mymethod} outperforms all other sparsification techniques across the Llama family.}
%         \label{tab:Llama_sparse_performance}
% \end{table}

\begin{table}[h!]
    \centering
        \caption{{\mymethod} across the Llama family. {\mymethod} outperforms all other sparsification techniques for every member of the Llama family.}
        \begin{tabular}{| l | c | c || c | c | c |} 
            \hline
            & Sparsity & Bits & Llama 2 7B & Llama 2 13B & Llama 2 70B\\
            \hline\hline
            Dense & 0\% & 16-bit & 5.1168 & 4.5736 & 3.3192 \\ 
            \hline
            MP & 50\% & 16-bit & 16.029 & 6.8270 & 4.9846\\
            Wanda & 50\% & 16-bit & 6.7757 & 5.8527 & 4.0219 \\
            SparseGPT & 50\% & 16-bit & 5.7082 & 5.0521 & 3.9013 \\
            \textbf{{\mymethod}} & 50\% & 16-bit & \textbf{5.5839} & \textbf{4.9728} & \textbf{3.8791}\\
            \hline
            SparseGPT & 2:4 & 16-bit & 6.9767 & 5.9934 & 4.8002\\
            \textbf{{\mymethod}} & 2:4 & 16-bit & \textbf{6.4456} & \textbf{5.6255} & \textbf{4.6671}\\
            \hline\
            SparseGPT & 2:4 & 4-bit & 7.2759 & 6.1101 & 4.9036 \\
            \textbf{{\mymethod}} & 2:4 & 4-bit & \textbf{6.5745} & \textbf{5.7151} & \textbf{4.7586} \\
            \hline
            SparseGPT & 2:4 & 3-bit & 13.076 & 6.5055 & 5.2552\\
            \textbf{{\mymethod}} & 2:4 & 3-bit & \textbf{7.0757} & \textbf{5.9872} & \textbf{5.0588}\\
            \hline
            
        \end{tabular}
        
        \label{tab:Llama_sparse_performance}
\end{table}


{\mymethod} outperforms all other pruning techniques for both 50\% unstructured sparsity as well 2:4 sparsity in all Llama models (Figure \ref{tab:Llama_sparse_performance}). In addition to non-quantized sparsity, we consider how {\mymethod} performs in the context of compression with 2:4 structured sparsity and quantization. We first sparsify each linear layer in each FFN block to 2:4 sparsity, then quantized to 3 and 4 bits. Our method outperforms SparseGPT across all models and across both conditions and in all models (Figure \ref{tab:Llama_sparse_performance}). 

Across multiple model sizes, sparsity and compression levels, and advanced models, {\mymethod} attains state-of-the-art performance for post-training one-shot sparsification when compared to other highly competitive pruning techniques. We do so by leveraging the powerful pruning algorithm of SparseGPT and combining it with input specialization to utilize the insights we gain from how entangled neurons behave under sparsity. 

% \begin{table}[h!]
%     \centering
%         \begin{tabular}{| l | c | c || c | c | c |} 
%             \hline
%              & Sparsity & Bits & Llama2-7B & Llama2-13B & Llama2-70B\\
%             \hline\hline
%             Dense & 0:4 & 16-bit & 5.1168 & 4.5736 & 3.3192\\ 
%             \hline
%             SparseGPT & 2:4 & 4-bit & 7.2759 & 6.1101 & 4.9036 \\
%             {\mymethod} & 2:4 & 4-bit & \textbf{6.5745} & \textbf{5.7151} & \textbf{4.7586} \\
%             \hline
%             SparseGPT & 2:4 & 3-bit & 13.076 & 6.5055 & 5.2552\\
%             {\mymethod} & 2:4 & 3-bit & \textbf{7.0757} & \textbf{5.9872} & \textbf{5.0588}\\
%             \hline
%         \end{tabular}
%         \caption{{\mymethod} outperforms SparseGPT in the Llama family under compression.}
%         \label{tab:Llama_compress_performance}
% \end{table}

% \begin{table}[h!]
%     \centering
%         \begin{tabular}{| l | c || c | c | c | c |} 
%             \hline
%              & Bits & Llama 2 7B & Llama 2 13B & Llama 2 70B & Llama 3 8B \\
%             \hline\hline
%             Dense & 16-bit & 5.1168 & 4.5736 & 3.1203 & 5.7503 \\ 
%             \hline
%             SparseGPT 2:4 & 4-bit & 7.2759 & 6.1101 & x & 88.730 \\
%             {\mymethod} 2:4 & 4-bit & \textbf{6.5745} & \textbf{5.7151} & x & \textbf{8.8090} \\
%             \hline
%             SparseGPT 2:4 & 3-bit & 13.076 & 6.5055 & RUNNING & 32.104 \\
%             {\mymethod} 2:4 & 3-bit & \textbf{7.0757} & \textbf{5.9872} & RUNNING & \textbf{11.193} \\
%             \hline
%         \end{tabular}
%         \caption{{\mymethod} outperforms SparseGPT in the Llama family under compression.}
%         \label{tab:Llama_compress_performance}
% \end{table}

% \begin{table}[h!]
%     \centering
%         \begin{tabular}{| l | c | c || c | c | c |} 
%             \hline
%              & Sparsity & Bits & Llama2-7B & Llama2-13B & Llama2-70B\\
%             \hline\hline
%             Dense & 0:4 & 16-bit & 5.1168 & 4.5736 & 3.3192\\ 
%             \hline
%             SparseGPT & 2:4 & 4-bit & 7.2759 & 6.1101 & 4.9036 \\
%             {\mymethod} & 2:4 & 4-bit & \textbf{6.5745} & \textbf{5.7151} & \textbf{4.7586} \\
%             \hline
%             SparseGPT & 2:4 & 3-bit & 13.076 & 6.5055 & 5.2552\\
%             {\mymethod} & 2:4 & 3-bit & \textbf{7.0757} & \textbf{5.9872} & \textbf{5.0588}\\
%             \hline
%         \end{tabular}
%         \caption{{\mymethod} outperforms SparseGPT in the Llama family under compression.}
%         \label{tab:Llama_compress_performance}
% \end{table}

% \subsection{Zero-shot Evaluation Performance}

% We assess {\mymethod} across five well-known zero-shot tasks:  WinoGrande \citep{sakaguchi2021winogrande}, HellaSwag \citep{zellers2019hellaswag}, ARC-e, and ARC-c \citep{clark2018think} and RTE . We used the default parameters of the LM Evaluation Harness \citep{eval-harness}, in line with previous work \citep{frantar2023sparsegpt, frantar2022gptq, dettmers2022gpt3}.

% \begin{table}[h!]
%     \centering
%         \begin{tabular}{| l | c | c | c | c | c | c | c |} 
%             \hline
%             & Sparsity & HellaSwag & WinoGrande & ARC-e & ARC-c & PIQA & Avg.\\
%             \hline\hline
%             Dense & 0\% & 75.99 & 69.53 & 76.30 & 46.33 & 79.16 & R \\ 
%             \hline
%             MP & 50\% & 65.69 & 63.54 & 64.14 & 37.46 & 73.67& R\\
%             Wanda & 50\% & 70.88 & 67.72 & 72.14 & 41.89 & 75.84 & R\\
%             SparseGPT & 50\% & 72.07 & 68.43 & 72.47 & 41.64 & 77.37 & R\\
%             {\mymethod} & 50\% & R & R & R & R & R & R\\
%             \hline
%         \end{tabular}
%         \caption{{\mymethod} outperforms all other sparsification techniques across various benchmarks.}
%         \label{tab:sparse_eval_performance}
% \end{table}



\subsection{Inference speed}
To evaluate the inference latency of {\mymethod} we implemented a {\mymethod} layer based on PyTorch and optimized sparse-quantized GPU kernels called Sparse Marlin \citep{frantar2024marlin, castro2024marlin}, which supports the INT4 + 2:4 sparse format. We use a linear layer of appropriate size as an upper bound approximation for our router cost, which is followed by 4 bits 2:4 sparse matrix multiplication. We have run the layer-wise benchmarks for the typical layers sizes from Llama models on a single RTX3090 GPU. 
We can see in Table~\ref{tab:inference_speed} that {\mymethod} allows us to get up to 4.8$\times$ speedup over the dense baseline. The speedup comes from the highly-compressed linear layer representation, while the overhead over the original kernels can be explained by the effect of interleaved calls of dense router and sparse experts during Sparse Expansion inference.

\begin{table}[h!]
    \centering
    \caption{{\mymethod} inference speedup. Layer-wise single batch inference latency (in $\mu$s). The layer sizes are chosen specifically to match the layers of Llama 2 7b and Llama 2 70B.}
    \begin{tabular}{|l||c|c|c|c|c|c|}
        \hline
        Layer Size & 4k $\times$ 12k & 4k $\times$ 22k & 11k $\times$ 4k & 8k $\times$ 10k & 8k $\times$ 57k & 28k $\times$ 8k \\
        \hline \hline
        Dense & 132 & 227 & 114 & 220 & 1168 & 556 \\
        \hline
        Sparse Expansion & 76 & 76 & 75 & 76 & 241 & 138 \\
        % \hline
        Speedup & 1.7$\times$ & 3.0$\times$ & 1.5$\times$ & 2.9$\times$ & 4.8$\times$ & 4.0$\times$ \\
        \hline
        Sparse & 26.8 & 44.7 & 24.4 & 42.3 & 216 & 109 \\
        % \hline
        Expansion Overhead & 2.9$\times$ & 1.7$\times$ & 3.1$\times$ & 1.8$\times$ & 1.1$\times$ & 1.3$\times$ \\
        \hline
    \end{tabular}
    
    \label{tab:inference_speed}
\end{table}




% \begin{table}[h!]
%     \centering
%     \begin{tabular}{c|c|c|c|c|c|c|}
%         \toprule
%         Layer Size & 4k $\times$ 12k & 4k $\times$ 22k & 11k $\times$ 4k & 8k $\times$ 10k & 8k $\times$ 57k & 28k $\times$ 8k \\
%         \midrule
%         Dense & 132 & 227 & 114 & 220 & 1168 & 556 \\
%         \midrule
%         Sparse Expansion & 76 & 76 & 75 & 76 & 241 & 138
%         \midrule
%         Speedup & 1.7 & 3.0 & 1.5 & 2.9 & 4.8 & 4.0  \\
%         \midrule
%         Sparse & 26.8 & 44.7 & 24.4 & 42.3 & 216.1 & 108.8 \\
%         \midrule
%         Expansion Overhead & 2.9 & 1.7 & 3.07 & 1.8 & 1.1 & 1.3 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Layer-wise single batch inference latency (in us). The layer sizes are chosen specifically to match the layers of LlaMa-7b and LlaMa-70B.}
%     \label{tab:inference_speed}
% \end{table}
% \shashata{Dan/Illia can you write this section?}
